Target-Driven Distillation: Consistency Distillation with Target Timestep Selection and Decoupled Guidance

Consistency distillation methods have demonstrated significant success in accelerating generative tasks of diffusion models. However, since previous consistency distillation methods use simple and straightforward strategies in selecting target timesteps, they usually struggle with blurs and detail losses in generated images. To address these limitations, we introduce Target-Driven Distillation (TDD), which (1) adopts a delicate selection strategy of target timesteps, increasing the training efficiency; (2) utilizes decoupled guidances during training, making TDD open to post-tuning on guidance scale during inference periods; (3) can be optionally equipped with non-equidistant sampling and x0 clipping, enabling a more flexible and accurate way for image sampling. Experiments verify that TDD achieves state-of-the-art performance in few-step generation, offering a better choice among consistency distillation models.

==> ann/sections/conclusion.tex <==
\section{Conclusion}

Consistency distillation methods have proven effective in accelerating diffusion models' generative tasks. However, previous methods often face issues such as blurriness and detail loss due to simplistic strategies in target timestep selection. We propose Target-Driven Distillation (TDD), which addresses these limitations by (1) employing a refined strategy for selecting target timesteps, thus enhancing training efficiency; (2) using decoupled guidance during training, which allows for post-tuning of the guidance scale during inference; and (3) incorporating optional non-equidistant sampling and $\mathbf{x}_0$ clipping for more flexible and precise image sampling. Experiments demonstrate that TDD achieves state-of-the-art performance in few-step generation, providing a superior option among consistency distillation methods.
\begin{figure}[t]
\centering
\includegraphics[width=.85\columnwidth]{AnonymousSubmission/LaTeX/x0_clip.pdf}
\caption{Ablation comparison of $\mathbf{x}_0 $ clipping sample. The prompt used is "a dog wearing a blue dress". The images on the left are with CFG=2, the middle with CFG = 3, and the right with CFG = 3 and $\mathbf{x}_0 $ clipping applied.}
\label{fig_x0_clip}
\vspace{-10pt}
\end{figure}

==> ann/sections/experiment.tex <==
\begin{table*}[h]
\centering

\label{tab:comparison_1}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{l|ccccc|ccccc}
\toprule
\multirow{3}{*}{METHOD} & \multicolumn{5}{c|}{FID $\downarrow$} & \multicolumn{5}{c}{Image Complexity Score $\uparrow$} \\ \cline{2-11} 
& \multicolumn{5}{c|}{COCO-30K} & \multicolumn{5}{c}{COCO-30K} \\ \cline{2-11} 
                        & 4 steps & 5 steps & 6 steps & 7 steps & 8 steps & 4 steps & 5 steps & 6 steps & 7 steps & 8 steps  \\ \hline
LCM & 18.424 & 18.906 & 19.457 & 19.929 & 20.494 
& 0.419 & 0.417 & 0.415  & 0.412 & 0.409\\
PCM & 22.213 & 21.921 & 21.916 & 21.786 & 21.772 & 0.433 & 0.447 & 0.458  & 0.465 & 0.471 \\
TCD & \underline{17.351} & \underline{17.430} & \underline{17.535} & \underline{17.65943} & \underline{17.771}
& \textbf{0.512} & \textbf{0.521} & \textbf{0.527}  & \textbf{0.533} & \textbf{0.536} \\
Ours & \textbf{17.256} & \textbf{17.388} & \textbf{17.334} & \textbf{17.565} & \textbf{17.681} 
& \underline{0.474} & \underline{0.488} & \underline{0.499} & \underline{0.508} & \underline{0.516}\\ \bottomrule
% \midrule
\toprule
%\toprule
\multirow{3}{*}{METHOD} & \multicolumn{10}{c} {PickScore $\uparrow$} \\ \cline{2-11}
& \multicolumn{5}{c|}{PartisPrompts} & \multicolumn{5}{c}{COCO-2K} \\ \cline{2-11}
                        & 4 steps & 5 steps & 6 steps & 7 steps & 8 steps & 4 steps & 5 steps & 6 steps & 7 steps & 8 steps  \\ \hline
LCM & 22.182 & 22.226 & 22.246 & 22.251 & 22.237 & 22.143 & 22.223 & 22.268 & 22.296 & 22.297\\
PCM & 22.200 & 22.289 & 22.340 & 22.357 & 22.367
& 22.291 & 22.433 & 22.505 & 22.537 & \underline{22.543}
\\
TCD & \textbf{22.350} & 22.402 & 22.417 & 22.426 & 22.426
& 22.310 & 22.423 & 22.490 & 22.504 & 22.504
\\
Ours & \underline{22.338} & \underline{22.414} & 22.445 & 22.472 & \textbf{22.493}
& \textbf{22.396} & \underline{22.533} & \underline{22.593} & \underline{22.640} & \textbf{22.656}
\\
Ours(*) & - & \textbf{22.431} & \textbf{22.472} & \textbf{22.489} 
& - & - & \textbf{22.577} & \textbf{22.630} & \textbf{22.652} & - \\
Ours(adv) & 22.279 & 22.388 & \underline{22.450} & \underline{22.476} & \underline{22.490} & \underline{22.322} & 22.466 & 22.502 & 22.511 & 22.508 \\
\bottomrule
\end{tabular}
}
\caption{Quantitative Comparison under different metrics and datasets.}
\end{table*}

\section{Experiments}


\subsection{Dateset}

We use a subset of the Laion-5B \cite{schuhmann2022laion} High-Res dataset for training. All images in the dataset have an aesthetic score above 5.5, totaling approximately 260 million.Additionally, we evaluate the performance using the COCO-2014 \cite{lin2014microsoft} validation set, split into 30k(COCO-30K) and 2k(COCO-2K) captions for assessing different metrics. We also use the PartiPrompts \cite{yu2022scaling} dataset to benchmark performance, which includes over 1600 prompts across various categories and challenge aspects.

\subsection{Backbone}
We employ SDXL \cite{podell2023sdxl} as the backbone for our experiments, specifically we trained a LoRA \cite{hu2021lora} through distillation.

\subsection{Metrics}
We evaluate image generation quality using Frechet Inception Distance (FID) \cite{heusel2017gans} and assess image content richness with the Image Complexity 
Score (IC) \cite{feng2022ic9600}. Additionally, we use Pickscore \cite{kirstain2023pick} to measure human preference. FID and IC are tested on the COCO-30K dataset, while PickScore is evaluated on COCO-2K and PartiPrompts.

\subsection{Performance Comparison}
In this section, we present a comprehensive performance evaluation of our proposed method against several baselines, including LCM, PCM, and TCD, across the COCO-30K, Parti Prompts, and COCO-2K datasets, as detailed in Table 1. We introduce two method, ``Ours" and ``Ours*", representing normal sampling and non-equidistant sampling (4-step and 8-step as normal sampling), respectively. Additionally, ``Ours(adv)" incorporates PCM's \cite{wang2024phased} adversarial process during distillation, demonstrating that our method can effectively integrate adversarial training.

As shown in \Cref{fig:main_res}, we qualitatively compare Ours and Ours(adv) with other methods across different inference steps. Our model outperforms others in image quality and text-image alignment, especially in the 4 to 8-step range. Quantitative results in  show that Ours achieves the best FID, though FID values tend to increase with more steps. While our method may not always achieve the top Image Complexity (IC), it avoids generating less detailed or cluttered images, unlike CTM, as seen in \Cref{fig:main_res}. However, the high image complexity observed in CTM may also be attributed to certain visual artifacts and high-frequency noise, which we will elaborate on in the appendix. Furthermore, evaluations using PickScore on the COCO-2K and PartiPrompt datasets show that Ours and Ours* consistently rank first or second in most cases. Overall, our method demonstrates superior performance and a well-balanced approach across metrics.

\subsection{Ablation Study}
\subsubsection{Effect of Target Timestep Selection}
To demonstrate the advantages of Target-Timestep-Selection, we compared the performance of models trained on mappings required for 4-step inference (i.e., PCM) against those trained on mappings required for 4-8 step inference. We maintained consistent settings with a batch size of 128, a learning rate of 5e-06, and trained for a total of 15,000 steps. As shown in \Cref{ab_tdd}, when using deterministic sampling (i.e., \(\gamma=0\)), the model trained on mappings for 4-8 step inference showed only a slight advantage at 4 and 5 steps. However, when incorporating randomness into sampling (i.e., \(\gamma=0.2\)), the model trained on 4-8 step mappings outperformed the model trained on 4-step mappings across all 4-8 steps. Furthermore, when we extended the mapping range by \(\eta=0.3\) to better accommodate the randomness in sampling (as indicated by the red line in \Cref{ab_tdd}), inference with \(\gamma=0.2\) achieved a well-balanced performance across 4-8 steps, avoiding poor performance at 4-5 steps while also maintaining solid performance at 6-8 steps.
\begin{figure}[t]
\centering
\includegraphics[width=0.85\columnwidth]{images/abs_2.pdf}
\caption{Qualitative comparison between Target-Driven Multi-Target Distillation (TDD, 4-8 step target timesteps distillation) and Single-Target Distillation (PCM, 4-step target timesteps distillation).}
\label{ab_tdd}
\end{figure}
\subsubsection{Effect of distillation with decoupled guidances and guidance scale tuning}
To demonstrate the advantages of distillation with decoupled guidances, we conducted experiments with a batch size of 128, \( K_{\text{min}} = 4 \), \( K_{\text{max}} = 8 \), and \(\eta = 0.3\), training two models with empty prompt ratios of 0 and 0.2. After 15k steps, we performed inference using a CFG of 3, as shown in \Cref{fig:abs} (b). This approach effectively stabilized image quality and reduced visual artifacts. Additionally, we applied the guidance scale tuning to models like TCD and PCM, which were distilled with higher CFG values (corresponding to original CFGs of 9 and 5.5, respectively, when inferred with CFG 1). Guidance scale tuning successfully converted these models to use normal CFG values during inference, significantly enhancing image content richness by reducing the CFG.
\begin{figure}[t]
    \centering
    \includegraphics[width=.85\linewidth]{images/abs.pdf}
    \caption{(a) Ablation comparison of distillation with decoupled guidances. (b) Ablation comparison of guidance scale tuning.}
    \label{fig:abs}
    \vspace{-10pt}
\end{figure}

\subsubsection{Effect of $\mathbf{x}_0$ clipping Sample}
In Figure 6, we demonstrate the advantages of \(\mathbf{x}_0\) clipping. For some samples inferred with a low guidance scale, such as the one on the far left, certain defects may appear during inference. Increasing the guidance can alleviate these issues to some extent, but it also increases contrast, as seen in the middle image of Figure 6. By applying clipping in the initial steps, we can partially correct these defects without increasing contrast. Additional examples and results from applying clipping beyond the first denoising step are provided in Appendix.

==> ann/sections/intro.tex <==
\section{Introduction}
Diffusion models \cite{sohl2015deep, song2019generative, karras2022elucidating} have demonstrated exceptional performance in image generation, producing high-quality and diverse images. Unlike previous models like GANs \cite{goodfellow2014generative, karras2019style} or VAEs \cite{kingma2013auto, sohn2015learning}, diffusion models are good at modeling complex image distributions, and conditioning on non-label conditions such as free-form text prompts.
% making them more effective for complex tasks like synthesizing images from free-form text descriptions. 
However, since diffusion models adopt iterative denoising processes, they usually take substantial time when generating images. To address such challenge, consistency distillation methods \cite{song2023consistency, luo2023latent, luo2023lcm, kim2023consistency, zheng2024trajectory, wang2024phased} have been proposed as effective strategies to accelerate generation while maintaining image quality.
These methods distill pretrained diffusion models following the \textit{self-consistency property} \textit{i.e.} the predicted results from any two neighboring timesteps towards the same target timestep are regularized to be the same. According to the choices of target timesteps, recent consistency distillation methods can be categorized as \textit{single-target distillation} and \textit{multi-target distillation}, illustrated in \Cref{fig:train_diff}.

Single-target distillation methods follow a one-to-one mapping when choosing target timesteps, that is, they always choose \textit{the same} target timestep each time they come to a certain timestep along the trajectory of PF-ODE \cite{song2020score}. One straightforward choice is mapping any timestep to the final timestep at 0 \cite{song2023consistency, luo2023latent}. However, these methods usually suffer from the accumulated error of long-distance predictions. Another choice is evenly partitioning the full trajectory into several sub-trajectories and mapping a timestep to the end of the sub-trajectory it belongs to \cite{wang2024phased}. Although the error can be reduced by shortening the predicting distances when training, the image quality will be suboptimal when adopting a schedule with a different number of sub-trajectories during inference periods.
% \cite{song2023consistency, luo2023latent, luo2023lcm, wang2024phased} assumes a fixed denoising step and a single denoising trajectory, mapping any data point at a given time to a target point at a determined timestep along the PF-ODE\cite{song2020score}.Typically, target points are determined by evenly dividing the time steps. As the number of segments increases, the effectiveness of distillation improves, but the number of denoising steps must match or exceed the number of segments. The challenge lies in balancing the number of segments with the need to train additional segments models to enhance generation quality, which increases the training burden.

On the other hand, multi-target distillation methods follow a one-to-multiple mapping, that is, \textit{possibly different} target timesteps may be chosen each time they come to a certain timestep. A typical choice is mapping the current timestep to a random target timestep ahead \cite{kim2023consistency, zheng2024trajectory}. Theoretically, these methods are trained to predict from any to any timestep, thus may generally achieve good performance under different schedules. Yet practically most of these predictions are redundant since we will never go through them under common denoising schedules. Hence, multi-target distillation methods usually require a high time budget to train.
% \cite{kim2023consistency, zheng2024trajectory} involves varying denoising steps and non-unique trajectories, allowing data points at any given time to map to different target points across timesteps. These methods aim to achieve anytime-to-anytime jumps, encompassing all possible denoising trajectories. While this approach significantly enhances the model's ability to generate diverse outputs, the majority of these trajectories are unnecessary during actual denoising, resulting in low distillation efficiency and insufficient focus on specific denoising steps.

%为了解决并进一步提升加速质量，我们xx
% To preserve as much of the teacher model's potential as possible while effectively targeting various few-step denoising trajectories, 
To mitigate the aforementioned issues, we propose \textbf{Target-Driven Distillation (TDD)}, a multi-target approach that emphasizes delicately selected target timesteps during distillation processes. Our method involves three key designs: 
\textbf{Firstly,} for any timestep, it selects a nearby timestep forward that falls into a few-step equidistant denoising schedule of a predefined set of schedules (\textit{e.g.} 4--8 steps), which eliminates long-distance predictions while only focusing on the timesteps we will probably pass through during inference periods under different schedules. Also, TDD incorporates a stochastic offset that further pushes the selected timestep ahead towards the final target timestep, in order to accommodate non-deterministic sampling such as \(\gamma\)-sampling \cite{kim2023consistency}.
% extra target points during training, ensuring balanced performance across sampling strategies.%均分不知道需不需要在这里写
\textbf{Secondly,} while distilling classifier-free guidance (CFG) \cite{ho2022classifier} into the distilled models, to align with the standard training process using CFG, TDD additionally replaces a portion of the text conditions with unconditional (\textit{i.e.} empty) prompts. With such a design, TDD is open to a proposed inference-time tuning technique on guidance scale, allowing user-specified balances between the accuracy and the richness of image contents conditioned on text prompts.
% TDD uses a fixed guidance scale and includes unguided empty prompts during guided distillation \cite{luo2023latent, meng2023distillation}. We consider the classifier-free guidance (CFG)\cite{ho2022classifier} strategy, which provides a more precise sample during training. Similar to standard diffusion model training \cite{rombach2022high}, it should also include a ratio of empty prompts to further enhance generation quality and text-image alignment. Additionally, we propose a Guided Inversion method that allows sampling with a normal guidance scale even after large CFG distillation, mitigating the loss of image richness due to CFG constraints.
\textbf{Finally,} TDD is optionally equipped with a non-equidistant sampling method doing short-distance predictions at initial steps and long-distance ones at later steps, which helps to improve overall image quality. Additionally, TDD adopts $\mathbf{x}_0$ clipping to prevent out-of-bound predictions and address the overexposure issue.
% 3) We propose N-sampling based on y-sampling, a non-equidistant sampling method. By not relying on a single set of equidistant points during training, we can adjust time steps to have smaller intervals at high noise levels and larger intervals at low noise levels, thereby enhancing generation quality. Additionally, to address overexposure issues caused by slightly larger CFG values in few-step sampling, we adopt an \(x_0\) formulation, enabling the clipping of \(x_0\) to prevent out-of-bound predictions during guided sampling with CFG.
% Single-Trajectory Distallaion and Multi-Trajectory Distallaion.
% Singlexxx multixxx,
% \begin{enumerate}
%     \item \textbf{Target-Driven Multi-Trajectory Distillation (TDMD)} We determine which target point a data point should estimate at a specific timestep based solely on commonly used denoising steps (e.g., 4-8 steps).Specifically, the distilled model retains the ability for a point at any timestep to estimate only a limited number of timesteps, ensuring that inference involves minimal redundant denoising trajectories while still supporting various denoising methods. Additionally, to accommodate random sampling, such as $\gamma$-sampling, we incorporate extra strategically selected target points during training. This ensures balanced performance across different sampling strategies.
%     \item \textbf{Guided Decoupled Distillation} TDD emphasizes using a fixed guidance coefficient and incorporating a proportion of unguided empty prompts during the CFG \cite{ho2022classifier} strategy in consistency distillation \cite{luo2023latent, meng2023distillation}. The CFG strategy provides a more precise sample during training without impacting inference. Similar to standard diffusion model training \cite{rombach2022high}, adding empty prompts enhances generation quality and text-image alignment. Additionally, we propose a Guided Inversion method based on the role of empty prompts in distillation, allowing sampling with a normal guidance scale even after large CFG distillation. This approach mitigates the reduction in image richness caused by CFG constraints during distillation.
%     \item \textbf{Sampling} We train a deep learning model using the preprocessed data.
% \end{enumerate}

% Diffusion model\cite{sohl2015deep, song2019generative} has demonstrated remarkable performance in image generation, producing high-quality and diverse images that significantly advance the capabilities and potential applications of generative models. Unlike GANs\cite{goodfellow2014generative} or VAEs\cite{kingma2013auto}, diffusion models rely on an iterative denoising process, enabling them to handle complex tasks such as synthesizing images from free-form text descriptions more effectively.However, this multi-step iteration requires substantial time and GPU resources, affecting user experience and incurring high costs.

% To address these challenges, consistency models\cite{song2023consistency}, especially those\cite{luo2023latent} distilled from a teacher model, or modules such as LCM-Lora\cite{luo2023lcm}, can achieve few-step generation with minimal retraining resources.These models all possess \textit{self-consistency} property: estimates for arbitrary pairs of points on the same PF-ODE trajectory \cite{song2020score} are consistent.For Consistency Models (CM), although the goal is to map any timestep directly to the initial point of the ODE trajectory (data sample) in one step, the learning difficulty increases for points further from timestep 0. This results in poor performance when mapping from pure noise in a single step. Consequently, while multi-step inference initially improves image quality, the benefits diminish as mapping performance deteriorates as the timestep approaches $T$, limiting further quality enhancement.

% CTM\cite{kim2023consistency} and TCD\cite{zheng2024trajectory} aims to enable consistency models to perform anytime-to-anytime jumps, allowing a point at any timestep to map to any point between timestep 0 and the previous timestep on the ODE trajectory. This approach reduces the mapping difficulty for each point and includes all possible jump-trajectories within the same ODE trajectory during training, enhancing generation diversity. However, it also includes many mappings that are irrelevant during actual inference, resulting in lower training efficiency.

% PCM\cite{wang2024phased} divides the ODE trajectory into multiple sub-trajectories, aiming for each point within a sub-trajectory to map to its initial point.  The more sub-trajectories there are, the lower the mapping difficulty for points further from the initial point, thus improving training efficiency.  Theoretically, this method only includes one jump trajectory during inference, which has an inference step that is the same as the number of sub-trajectories.  If we use a model divided into 4 sub-trajectories to generate a preferred image and want higher quality, we must use models divided into 5, 6, or more steps.  This increases the training burden and makes model switching in real applications less user-friendly.  Another approach is to double the number of inference steps so that each jump remains within the range of a sub-trajectory.  However, this is less flexible, significantly increases inference time, and without additional mappings, cannot achieve the same quality as a model with double the sub-trajectories.

% This paper, we introduce TDD, which allows for flexible and accurate selection of different jump trajectories on the same ODE trajectory using a single model for few-step inference.Specifically, we enable any point on the same PF-ODE trajectory to map to a finite set of strategically selected points based on the desired few-step inference range and the point's position on the trajectory. This ensures that during inference, the mappings can be precisely utilized without redundancy. Unlike approaches that focus on a single jump trajectory during training (with each point having a unique, determined mapping) or those considering all possible jump trajectories (with each point having every possible mapping), TDD includes only the necessary specific jump trajectories for few-step sampling. This approach enhances the efficiency of deterministic sampling while allowing for flexible selection of different inference steps, thereby optimizing generation quality.Moreover, another advantage of TDD is its ability to perform non-equidistant jumps. By increasing the number of jumps at larger timesteps, TDD enhances detail while keeping the total number of steps unchanged.

% Additionally, TDD emphasizes using a fixed guidance coefficient and incorporating a proportion of unguided empty prompts during the CFG\cite{ho2022classifier} strategy in consistency distillation\cite{luo2023latent, meng2023distillation}.
% We consider that the CFG strategy provides a more precise sample during training, which does not affect its use during inference. Similar to standard diffusion model training\cite{rombach2022high}, adding a ratio of empty prompts further enhances generation quality and text-image alignment.This advantage is more pronounced in high CFG settings.To further leverage this, we adapted \(\gamma\)-sampling \cite{kim2023consistency} to an \(x_0\) formulation, enabling the clipping of \(x_0\) to prevent out-of-bound predictions during guided sampling with CFG.

Our contributions are summarized as follows:
\begin{itemize}
    \item We provide a taxonomy on consistency distillation models, classifying previous works as \textit{single-target} and \textit{multi-target} distillation methods.
    \item We propose Target-Driven Distillation, which highlights target timestep selection during distillation processes.
    \item We present extensive experiments to validate the effectiveness of our proposed distillation method.
\end{itemize}
% \begin{itemize}
%     \item \textbf{Flexible Accelerate}
%      We propose TDD for flexible and accurate selection of jump trajectories, allowing non-equidistant jumps to enhance detail without increasing steps, optimizing image quality.
%     \item \textbf{Sample}
%     We use a fixed guidance coefficient and unguided empty prompts during consistency distillation, along with
%     \item \textbf{Performance:}??.
% \end{itemize}

\begin{figure}[t]
\centering
\includegraphics[width=1.\columnwidth]{images/train_diff_2.pdf} 
\caption{Comparison of different distillation methods. $ \tau^{k_1}_m $ and $ \tau^{k_2}_m $ represent a target timestep when divided into $k_1$ and $k_2$, respectively. LCM (a) and PCM (b) are examples of single-target distillation, where $ \mathbf{x}_{t_{n}} $ corresponds to only one target timestep. In contrast, CTM (c) and ours (d) are multi-target distillation methods, where $ \mathbf{x}_{t_{n}} $ can correspond to multiple target timesteps.}
\label{fig:train_diff}
\end{figure}


==> ann/sections/method.tex <==
\section{Method}

In this section, we will first deliver some preliminaries in \cref{sec:pre}, followed by detailed descriptions of our proposed Target-Driven Distillation in \Cref{sec:select,sec:cfg,sec:sample}.
% In this section, we introduce TDD, an optimized consistency distillation strategy. 
% First, First, we analyze previous methods and present a unified distillation loss formula for consistency models.
% Next, we propose Target-Driven Multi-Trajectory Distillation to accelerate generation. Additionally, we describe the use of Guided Decoupled Distillation in the process and present the Guided Inversion method. Finally, we introduce N-Sampling, which further enhances the quality of few-step generation.

\subsection{Preliminaries}
\label{sec:pre}

\subsubsection{Diffusion Model}
Diffusion models constitute a category of generative models that draw inspiration from thermodynamics and stochastic processes, encompass both a forward process and a reverse process.
The forward process is modeled as a stochastic differential equation (SDE) \cite{song2020score, karras2022elucidating}. Let \( p_{\text{data}}(\mathbf{x}) \) denotes the data distribution and \( p_t(\mathbf{x}) \) the distribution of \(\mathbf{x}\) at time $t$. For a given set \(\{\mathbf{x}_t | t \in [0, T]\}\), the stochastic trajectory is described by:
\begin{equation}
\mathrm{d}\mathbf{x}_t = f(\mathbf{x}_t, t) \, \mathrm{d}t + g(t) \, \mathrm{d}\mathbf{w}_t,
\label{eq:1}
\end{equation}
where \( \mathbf{w}_t \) represents standard Brownian motion, \( f(\mathbf{x}_t, t) \) is the drift coefficient for deterministic changes, and \( g(t) \) is the diffusion coefficient for stochastic variations. At \( t = 0 \), we have \( p_0(\mathbf{x}) \equiv p_{\text{data}}(\mathbf{x}) \).

% Specifically, the forward process can be described as a stochastic differential equation (SDE) \cite{song2020score, karras2022elucidating}. Define \( p_{\text{data}}(\mathbf{x}) \) as the data distribution and \( p_t(\mathbf{x}) \) as the distribution of \(\mathbf{x}_t\). For a given set \(\{\mathbf{x}_t\}_{t=0}^T\), with \( t \in [0, T] \), the realization of a stochastic trajectory can be expressed by the following equation:
% \begin{equation}
% d\mathbf{x}_t = f(\mathbf{x}_t, t) \, dt + g(t) \, d\mathbf{w}_t
% \label{eq:1}
% \end{equation}
% where \( \mathbf{w}_t \) represents standard Brownian motion, while \( f(\mathbf{x}_t, t) \) is the drift coefficient for deterministic changes, and $ g(t) $ is the diffusion coefficient for stochastic variations.  At \( t = 0 \), we have \( p_0(\mathbf{x}) \equiv p_{\text{data}}(\mathbf{x}) \).

Any diffusion process described by an SDE can be represented by a deterministic process described by an ODE that shares identical marginal distributions, referred to as a Probability Flow ODE (PF-ODE). The PF-ODE is formulated as:
\begin{equation}
\mathrm{d}\mathbf{x} = \left[ f(\mathbf{x}, t) - \frac{1}{2}g(t)^2 \nabla_{\mathbf{x}} \log p_t(\mathbf{x}) \right] \mathrm{d}t,
\label{eq:pfode}
\end{equation}
where $ \nabla_{\mathbf{x}} \log p_t(\mathbf{x}) $ represents the gradient of the log-density of the data distribution $p_t(\mathbf{x})$, known as the score function. 
Empirically, we approximate this score function with a score model $ s_\phi(\mathbf{x}, t)$ trained via score matching techniques. Although there are numerous methods \cite{song2020denoising, lu2022dpm, lu2022dpm++, karras2022elucidating} available to solve ODE trajectories, they still necessitate a large number of sampling steps to attain high-quality generation results.

\subsubsection{Consistency Distillation}

To render a unified representation across all consistency distillation methods, we define the teacher model as $\phi$, the consistency function with the student model as $ \boldsymbol{f}_{\theta} $, the conditional prompt as $ c $, and the ODE solver $ \Phi(\cdots; \phi) $ predicting from a certain timestep $t_{n+1}$ to its previous timestep $t_n$ following an equidistant schedule from $T$ to $0$.
% with $ T $ representing the total training timesteps for $ T_\phi $ and $ N $ the total distillation timesteps for the student model. The time interval for each skip step using $ \Phi(\cdot, \cdot, \cdot) $ is $ h = T/N $. The trajectory point at time $ t $ is denoted by $ \mathbf{x}_t $, where $ t_0 < t_1 < \cdots < t_N = T $ and $ t_{n+1} - t_n = h $. Here, $ n $ is uniformly distributed over the set $ \{0, 1, \ldots, N-1\} $.
With a certain point $\mathbf{x}_{t_{n+1}}$ on the trajectory at timestep $t_{n+1}$, and its previous point $\hat{\mathbf{x}}^{\phi}_{t_n}$ predicted by $\Phi(\cdots; \phi)$, the core consistency loss can be formulated as
% For an accurate estimate $\hat{\mathbf{x}}^{\phi}_{t_n}$ from $\mathbf{x}_{t_{n+1}}$ updated by $\Phi(\mathbf{x}_{t_{n+1}}, t_{n+1}, t_n; T_\phi)$, the loss function for all consistency distillation methods can be expressed in a unified form as follows:
\begin{equation}
\mathcal{L}_{\text{CMs}}:= 
    \left\| \boldsymbol{f}_{\theta}(\mathbf{x}_{t_{n+1}}, t_{n+1}, \tau) - \boldsymbol{f}_{\theta^{-}}(\hat{\mathbf{x}}_{t_n}^{\phi}, t_n, \tau) \right\|_2^2,
\end{equation}
where $ \boldsymbol{f}_{\theta^{-}} $ is the consistency function with a target model updated with the exponential moving average (EMA) from the student model, and $\tau$ refers to the \textit{target timestep}. 

Among the mainstream distillation methods, the choices of $\tau$ are the most critical differences (see \Cref{fig:train_diff}). Single-target distillation methods select the same $\tau$ each time when predicting from a certain $t_{n+1}$. For example, CM \cite{song2023consistency} sets $\tau = 0$ for any timestep $t_{n+1}$, while PCM \cite{wang2024phased} segments the full trajectory into $\mathcal{K}$ (\textit{e.g.} 4) phased sub-trajectories, and chooses the next ending point:
\begin{equation}
    \tau = \max \left\{\tau \in \{{0, {\frac{T}{\mathcal{K}}}, {\frac{2T}{\mathcal{K}}}, \ldots, {\frac{(\mathcal{K}-1)T}{\mathcal{K}}} }\} \mid \tau < t_n\right\}.
\end{equation}
On the other hand, multi-target distillation methods may select different values for $\tau$ each time predicting from $t_{n+1}$. For instance, CTM \cite{kim2023consistency} selects a random $\tau$ within the interval $[0, t_n]$.

% From the perspective of the selection of consistency-target-timestep, we define the following. For \textit{Single-Trajectory Distillation}: each adjacent pair $ (t_n, t_{n+1}) $ corresponds to a single $ \tau $. For \textit{Multi-Trajectory Distillation}: each adjacent pair $ (t_n, t_{n+1}) $ can correspond to multiple $ \tau $.
Our TDD, different from previous approaches that rely on simple trajectory segmentation or selecting from all possible $\tau$, we employ a strategic selection of $\tau$, detailed in \cref{sec:select}. According to the taxonomy we provide in this work, TDD is a multi-target distillation method, yet we strive to reduce training on redundant predictions that are unnecessary for inference. 
% The distinctions between our distillation method and the existing approaches are illustrated in \Cref{fig:train_diff}, and our sampling method is detailed in \Cref{fig:sample}.

% For an accurate estimate $\hat{\mathbf{x}}^{\phi}_{t_n}$ from $\mathbf{x}_{t_{n+1}}$ updated by $\Phi(\mathbf{x}_{t_{n+1}}, t_{n+1}, t_n; T_\phi)$, the CM (xx)loss is defined as:
% \begin{equation}
% \mathcal{L}_{\text{CM}}:= 
%     \left\| \boldsymbol{f}_{\theta_{S}}(\mathbf{x}_{t_{n+1}}, t_{n+1}, 0) - \boldsymbol{f}_{\theta_{S}^{-}}(\hat{\mathbf{x}}_{t_n}^{\phi}, t_n, 0) \right\|_2^2
% \end{equation}
% where $f_{\theta_{S}^{-}}$ is and the boundary timestep for consistency models is fixed at 0. However, the boundary timestep $ t_{s} $ for CTM is variable and can take any value within the interval $ [0, t_n] $.The loss can be expressed as follow:
% \begin{equation}
% \mathcal{L}_{\text{CTM}}:= 
%     \left\| \boldsymbol{f}_{\theta_{S}}(\mathbf{x}_{t_{n+1}}, t_{n+1}, t_s) - \boldsymbol{f}_{\theta_{S}^{-}}(\hat{\mathbf{x}}_{t_n}^{\phi}, t_n, t_s) \right\|_2^2
% \end{equation}
% PCM can be viewed as a segmented version of CM, divided into $\mathcal{K}$ segments(usually $\mathcal{K}=4$) based on the desired number of inference steps after distillation.
% \begin{equation}
% \mathcal{L}_{\text{PCM}}:= 
%     \left\| \boldsymbol{f}_{\theta_{S}}(\mathbf{x}_{t_{n+1}}, t_{n+1}, t_k) - \boldsymbol{f}_{\theta_{S}^{-}}(\hat{\mathbf{x}}_{t_n}^{\phi}, t_n, t_k) \right\|_2^2
% \end{equation}
% where $k \in \{{0, {\frac{N}{\mathcal{K}}}, {\frac{2N}{\mathcal{K}}}, \ldots, {\frac{(\mathcal{K}-1)N}{\mathcal{K}}} }\}$ and $t_k$ is the closest value to $t_n$ with $t_k < t_n$.

% Our method, TDD, differs from the aforementioned distillation approaches by focusing on commonly used endpoints while enhancing robustness. The distinctions between our distillation method and the existing approaches are illustrated in \cref{fig:train_diff}, and our sampling method is detailed in \cref{fig:sample}.

\subsection{Target Timestep Selection}
\label{sec:select}

First, TDD pre-determines a set of equidistant denoising schedules, whose numbers of denoising steps range from $\mathcal{K}_{\min}$ to $\mathcal{K}_{\max}$, that we may adopt during inference periods. In the full trajectory of a PF-ODE from $T$ to $0$, for each $k \in [\mathcal{K}_{\min}, \mathcal{K}_{\max}]$, the corresponding schedule include timesteps $\{\tau_m^k\}_{m = 0}^{k - 1}$ where $\tau_m^k = \frac{mT}{k}$. Then, we can define the union of all the timesteps of these schedules as 
\begin{equation}
\label{eq:T}
    \mathcal{T} = \bigcup_{k=\mathcal{K}_{\min}}^{\mathcal{K}_{\max}} \{\tau_m^k\}_{m = 0}^{k - 1},
\end{equation}
which includes all the possible timesteps that we may choose as target timesteps. Note that \Cref{eq:T} is a generalized formulation, where $\mathcal{K}_{\min}=\mathcal{K}_{\max}=1$ for CM, $1 < \mathcal{K}_{\min}=\mathcal{K}_{\max} < N$ for PCM, and $\mathcal{K}_{\min}=\mathcal{K}_{\max}=N$ for CTM where $N$ is the total number of predictions within the equidistant schedule used by the ODE solver $\Phi$. As for our TDD, we cover commonly used few-step denoising schedules. For instance, typical values for $\mathcal{K}_{\min}$ and $\mathcal{K}_{\max}$ are respectively $4$ and $8$.
% the selection set of consistency target timesteps based on a range of expected denoising steps, denoted by .
% For a solution trajectory of a diffusion model $\{\mathbf{x}_t\}_{t \in [\epsilon, T]} $ following the PF-ODE and one denoising trajectory over $ k $ steps ( $\mathcal{K}_{\min} \leq k \leq \mathcal{K}_{\max}$ ) denoted as $ \{\mathbf{x}_{\tau^k_m} \} $, we have $ \tau^k_m \in \{ \tau^k_0, \tau^k_1, \ldots, \tau^k_{k-1} \} $. For the same $ k $, the time intervals of the trajectory are evenly divided, given by $ \Delta{t} = \frac{T}{k}$. Thus, we have $ \{\mathbf{x}_{\tau^k_m} \mid k \in [\mathcal{K}_{\min}, \mathcal{K}_{\max}], m \in [0, k-1]\}$ representing the trajectories for all desired denoising steps.Specifically, when $\mathcal{K}_{\min}=\mathcal{K}_{\max}$, we obtain PCM; when $\mathcal{K}_{\min}=\mathcal{K}_{\max}=1$, it corresponds to CM; and when $
% \mathcal{K}_{\min}=1 $ and $ \mathcal{K}_{\max}=N $, it corresponds to CTM.
% we consider dividing the trajectory into $ k $ sub-trajectories, where $ k $ is an integer within a specified range (e.g., $4 \leq k \leq 8$), representing the number of inference steps required after distillation.$\tau^\mathcal{K}_n $These sub-trajectories have boundary time steps $\tau_{k, 0}, \tau_{k, 1}, \ldots, \tau_{k, \mathcal{K}}$, with $k$ indicating the sub-trajectory index, $\mathcal{K}_{\min} \leq k \leq \mathcal{K}_{\max}$, where $\tau_{k, 0} = \epsilon$ and $\tau_{k, \mathcal{K}} = T$. 
% For a solution trajectory of a diffusion model $\{\mathbf{x}_t\}_{t \in [\epsilon, T]} $ following the PF-ODE, we consider dividing the trajectory into $ k $ sub-trajectories, where $ k $ is an integer within a specified range (e.g., $4 \leq \mathcal{K} \leq 8$), representing the number of inference steps required after distillation.$\tau^\mathcal{K}_n $These sub-trajectories have boundary time steps $\tau_{k, 0}, \tau_{k, 1}, \ldots, \tau_{k, \mathcal{K}}$, with $k$ indicating the sub-trajectory index, $\mathcal{K}_{\min} \leq k \leq \mathcal{K}_{\max}$, where $\tau_{k, 0} = \epsilon$ and $\tau_{k, \mathcal{K}} = T$. 

% For any given sub-trajectory $k$ with \( t \in [\tau_{k, n}, \tau_{k, n+1}] \) the output boundary conditions should consistently remain the same.
Based on the condition, we establish the consistency function as:
\begin{equation}
 \boldsymbol{f}: (\mathbf{x}_t, t, \tau) \mapsto \mathbf{x}_{\tau} 
 \label{eq:tddfc}
\end{equation}
where \( t \in [0, T] \) and $ \tau \in \mathcal{T}$, and we expect that the predicted results to the specific target timestep $\tau$ will be consistent.

% In the context of the same inference path $k$, adhering to the PF-ODE, we require that the endpoints at any times \( t, t' \in [\tau_{k, n}, \tau_{k, n+1}] \) remain consistent, i.e.,\( f^{k, n} (\mathbf{x}_t, t) =  f^{k, n} (\mathbf{x}_{t'}, t')\).As depicted in Figure xx, the consistency function \(f^{k}\) across multiple $\mathcal{K}$ paths are learned using the consistency model \(f_\theta\).

\subsubsection{Training}
Although $\mathcal{T}$ is already a selected set of timesteps, predicting to an arbitrary timestep in $\mathcal{T}$ still introduces redundancy, as it is unnecessary for the model to learn long-distance predictions from a large timestep $t$ to a small $\tau$ in the context of few-step sampling. Therefore, we introduce an additional constraint $ e = \frac{T}{\mathcal{K}_{\min}} $. This constraint further narrows possible choices at timestep $t$, reducing the learning difficulty.
Formally, we uniformly select
\begin{equation}
    \tau_m \sim \mathcal{U}(\{\tau \in \mathcal{T} | t - e \leq \tau \leq t\}).
\end{equation}
Besides, $\gamma$-sampling  \cite{kim2023consistency} is commonly used in few-step generation to introduce randomness and stabilize outputs. To accommodate this, we introduce an additional hyperparameter $\eta \in [0, 1]$. The final consistency target timesteps are selected following 
\begin{equation}
    \tilde{\tau}_{m} \sim \mathcal{U}([{(1-\eta){\tau}_{m}}, {\tau}_{m}]).
\end{equation}

Define the solution using the master teacher model $T_\phi$ from $ \mathbf{x}_{t_{n+1}} $ to $ \mathbf{x}_{t_{n}} $ with PF ODE solver as follows:
\begin{equation}
\hat{\mathbf{x}}^{\phi}_{t_n} = \Phi(\mathbf{x}_{t_{n+1}}, t_{n+1}, t_n; T_\phi),
\label{eq:xtq}
\end{equation}
where \( \Phi(\cdot \cdot \cdot; T_\phi) \) is update function and $ \hat{\mathbf{x}}^{\phi}_{t_n} $ is an accurate estimate of $ \mathbf{x}_{t_{n}} $ from $ \mathbf{x}_{t_{n+1}} $.
The loss function of TDD can be defined as:

\begin{equation}
\begin{aligned}
\mathcal{L}_{\text{TDD}}(\theta, \theta^{-}; \phi) := E[\sigma(t_n, \tilde{\tau}_{m})
    &\left\| \boldsymbol{f}_\theta(\mathbf{x}_{t_{n+1}}, t_{n+1}, \tilde{\tau}_{m}) \right. \\
    &\left. - \boldsymbol{f}_{\theta^{-}}(\hat{\mathbf{x}}_{t_n}^{\phi}, t_n, \tilde{\tau}_{m}) \right\|_2^2],
\end{aligned}
\end{equation}
where the expectation is over $\mathbf{x} \sim p_{\text{data}}$, $n \sim {\mathcal{U}}[1, N-1]$, $\mathbf{x}_{t_{n+1}} \sim \mathcal{N}(\mathbf{x}; t_{n+1}^2 I)$ and $\hat{\mathbf{x}}_{t_n}^{\phi}$ is defined by \Cref{eq:xtq}.Namely, ${\mathcal{U}}[1, N-1]$ denotes a uniform distribution over 1 to $N-1$, where $N$ is a positive integer. $\sigma(\cdot, \cdot)$ is a positive weighting function, following CM, we set \( \sigma(t_n, \tilde{\tau}_{m}) \equiv 1 \). For a detailed description of our algorithm, please refer to \Cref{alg:gtcd}.

\begin{algorithm}[tb]
\caption{TDD Distillation}
\label{alg:gtcd}
\textbf{Input}: dataset $\mathcal{D}$, , learning rate $\delta$, the update function of ODE solver \( \Phi(\cdot \cdot \cdot; \cdot) \), EMA rate $\mu$, noise schedule $\alpha_t, \sigma_t$, number of ODE steps $N$, fixed gudiance scale $\omega'$, empty prompt ratio $\rho$.\\
\textbf{Parameter}: initial model parameter $\theta$\\
\textbf{Output}:
\begin{algorithmic}[1] %[1] enables line numbers
\STATE \(\mathcal{T} \gets \emptyset\)
\FOR{$k \in \{\mathcal{K}_{\min}, \mathcal{K}_{\min}+1, \ldots, \mathcal{K}_{\max}\}$}
\STATE Set time steps $\tau^k_m \in \{ \tau^k_0, \tau^k_1, \ldots, \tau^k_{k-1} \}$
\STATE Add time steps to $\mathcal{T}$
\ENDFOR
\STATE let $e = \frac{T}{\mathcal{K}_{\min}}$
% \STATE let \(
% \mathcal{T} = \operatorname{sort}(\operatorname{unique}(\mathcal{T}))
% \)
\REPEAT
\STATE Sample $(z, c) \sim \mathcal{D}, \tau_m \sim \mathcal{U}(\{\tau \in \mathcal{T} | t - e \leq \tau \leq t\})$
\STATE Sample $n \sim \mathcal{U}[1, N - 1], \tilde{\tau}_{m} \sim \mathcal{U}([{(1-\eta){\tau}_{m}}, {\tau}_{m}])$

\STATE Sample $\mathbf{x}_{t_{n+1}} \sim \mathcal{N}(\alpha_{t_{n+1}} \mathbf{x}, \sigma_{t_{n+1}}^2 \mathbf{I})$
\IF{probability $>$ $\rho$}
    \STATE $\begin{aligned}\hat{\mathbf{x}}^{\phi, w'}_{t_n} \gets &(1 + \omega') \Phi(\mathbf{x}_{t_{n+1}}, t_{n+1}, t_n, c; T_\phi) \\
& - \omega' \Phi(\mathbf{x}_{t_{n+1}}, t_{n+1}, t_n; T_\phi)\end{aligned}$
\ELSE
    \STATE $\hat{\mathbf{x}}^{\phi, w'}_{t_n} \gets \Phi(\mathbf{x}_{t_{n+1}}, t_{n+1}, t_n;T_\phi)
    $
\ENDIF
\STATE 
$
\mathcal{L}^{w'}_{\text{TDD}}:= 
    \left\| \boldsymbol{f}_{\theta}(\mathbf{x}_{t_{n+1}}, t_{n+1}, \tilde{\tau}_{m}) - \boldsymbol{f}_{\theta^{-}}(\hat{\mathbf{x}}^{\phi, w'}_{t_n}, t_n, \tilde{\tau}_{m}) \right\|_2^2
$
\STATE $\theta \gets \theta - \delta \nabla_{\theta} \mathcal{L}(\theta, \theta^-; \phi)$
\STATE $\theta^- \gets \text{sg}(\mu \theta^- + (1 - \mu) \theta)$
\UNTIL convergence
\end{algorithmic}
\end{algorithm}

\begin{figure}[t]
\centering
\includegraphics[width=1.\columnwidth]{images/sample_fin.pdf}
\caption{Illustration of TDD distillation training and sampling processes. Fig (a) shows the distillation process, where $\tau^{k}$ represents equidistant timestep within segments. Fig (b) compares non-equidistant sampling with standard sampling for 5-step inference.}

\label{fig:sample}
\end{figure}

\subsection{Guidances Decoupled}
\label{sec:cfg}

\subsubsection{Distillation with Decoupled Guidances}
Classifier-Free Guidance allows a model to precisely control the generation results without relying on an external classifier during the generation process, effectively modulating the influence of conditional signals. In current consistency model distillation methods, to ensure the stability of the training process, it is common to use the sample \(\hat{\mathbf{x}}^{\phi, w'}_{t_n}\) generated by the teacher model with classifier-free guidance as a reference in the optimization process for the student model's generated samples. We believe that $w'$ solely represents the diversity constraint in the distillation process, controlling the complexity and generalization of the learning target. This allows for faster learning with fewer parameters. Therefore, $w'$ should be treated separately from the CFG scale $w$ used during inference in consistency models. Therefore, regardless of whether $w' > 0$, following \cite{ho2022classifier}, it is essential to include both unconditional and conditional training samples in the training process.
Based on this, we will replace a portion of the condition with an empty prompt and not apply CFG enhancement. For conditions that are not empty, the loss function of TDD can be updated as follows:
\begin{equation}
    \mathcal{L}^{w'}_{\text{TDD}}:= 
    \left\| \boldsymbol{f}_{\theta}(\mathbf{x}_{t_{n+1}}, t_{n+1}, \tau) - \boldsymbol{f}_{\theta^{-}}(\hat{\mathbf{x}}^{\phi, w'}_{t_n}, t_n, \tau) \right\|_2^2.
\end{equation}

\begin{figure*}[t]
\centering
\includegraphics[width=2.0\columnwidth]{images/main_fig.pdf}
\caption{Qualitative comparison of different methods under NEF for 4 to 8 steps.}
\label{fig:main_res}
\end{figure*}

\subsubsection{Guidance Scale Tuning}
Define $\epsilon_\theta(\mathbf{x}_t)$ as consistency model, at each inference step, the noise predicted by the model can be expressed as:
\begin{equation}
  \hat{\epsilon_w} = (1 + {w})\epsilon_\theta({\mathbf{x}}^{w'}_{t}, t, c) - {w}\epsilon_\theta({\mathbf{x}}^{w'}_{t}, t),
\end{equation}
where ${\mathbf{x}}^{w'}_{t}$ represents the input state of the consistency model at time step $t$ distilled with the diversity guidance scale $w'$.

Although setting a high value for $w'$ (e.g., $w' > 7$) can enhance certain aspects of the generated images, it simultaneously results in significantly reduced image complexity and excessively high contrast.

Is there a way to address this issue without retraining, allowing us to revert to results that enable inference with a small CFG, similar to the original model? By incorporating the unconditional into the training, we can get $
\epsilon_\theta({\mathbf{x}}^{w'}_{t}, t, c) \propto (1 + {w'})\epsilon_\phi({\mathbf{x}}_{t}, t, c) - {w'}\epsilon_\phi({\mathbf{x}}_{t}, t) 
$ and  $\epsilon_\theta({\mathbf{x}}^{w'}_{t}, t) \propto \epsilon_\phi({\mathbf{x}}_{t}, t)
$, where $\epsilon_\phi(*)$ is the master model.

Denote \((1+w)\epsilon_\phi({\mathbf{x}}_{t}, t, c)-w\epsilon_\phi({\mathbf{x}}_{t}, t)\) as $\epsilon_{w}$, representing the noise inferred by the original model when using the normal guidance scale $ w $ at each time step. After simplification, we finally obtain:
\begin{equation}
    \epsilon_{w} \approx [\hat{\epsilon_w} + {w'}\epsilon_\theta({\mathbf{x}}_{t}, t)]/(1+{w'}).
\end{equation}
This equation suggests that regulating \( \hat{\epsilon_w} \) with the normal $w$ can approximate the output of the original model $ \epsilon_{w} $.For a more detailed derivation, please refer to the appendix.

In the aforementioned formula, the distillation diversity constraint $w'$ is known and fixed. The parameter $w$ can be inferred based on the standard teacher model's ratio. Furthermore, for the current consistency model, even though it has not yet learned the unguided path, this formula can still be approximately utilized for inference, as no other learning has been conducted. This can be expressed as follows:
\begin{equation}
    \epsilon'_{w} \approx [\hat{\epsilon'_w} + \overline{w'}\epsilon'_\theta({\mathbf{x}}_{t}, t)]/(1+\overline{w'}).
\end{equation}
where $\epsilon'_\theta(*)$ is current consistency model and $\overline{w'}= {w'_{min} + w'_{max})/2}$.

\subsection{Sample}
\label{sec:sample}
Since we have trained on multiple equidistant target timesteps, we can extend this to non-equidistant sampling. As shown in \Cref{fig:sample} (a), we ensure that the inference process passes through the target timesteps corresponding to $ \mathcal{K}_{\min} $. As the inference steps increase, additional target timesteps are gradually inserted between these key timesteps. For example, with $ \mathcal{K}_{\min}=4 $, as the number of steps increases, we insert 8-step ($ \mathcal{K}_{\max} $) target timesteps within each adjacent 4-step target interval to enhance generation quality.

In addition, the $\gamma$-sampler proposed in CTM \cite{kim2023consistency} alternates forward and backward jumps along the solution trajectory to solve \(\mathbf{x}_0\), allowing control over the randomness ratio through $\gamma$, which can enhance generation quality to some extent. Solving for $\mathbf{x}_s$ from $\mathbf{x}_t$ can be represented as follows:
\begin{equation}
\mathbf{x}_s = \frac{\alpha_s}{\alpha_t} \mathbf{x}_t - \sigma_s \left(e^{h_s} - 1\right) \epsilon_\theta(\mathbf{x}_t, t)
\end{equation}
where $h_s=\lambda_s - \lambda_t$ and $\lambda$ represents the log signal-to-noise ratio, $\lambda=log(\alpha/\sigma)$.However, in few-step sampling with high CFG inference, the noise distribution after the first step significantly deviates from the expected distribution. To address this, we adopt an \(\mathbf{x}_0\) formulation.To approximate $x_\theta(x_t, t) \approx x_0 = (\mathbf{x}_t - \sigma_t \epsilon)/(\alpha_t)$, , we can derive:
\begin{equation}
    \mathbf{x}_s = \frac{\sigma_s}{\sigma_t} \mathbf{x}_t - \alpha_s \left(e^{-h_s} - 1\right)x_\theta(\mathbf{x}_t, t)
\end{equation}
As shown in \Cref{fig:sample} (b), following prior works \cite{saharia2022photorealistic, lu2022dpm++}, we apply the clipping method $\mathcal{C}$, which clips each latent variable to the specific percentile of its absolute value and normalizes it to prevent saturation of the latent variables.
Let $\hat{\mathbf{x}_0}=\mathcal{C}(x_\theta(\mathbf{x}_t, t))$, we ultimately obtain:
\begin{equation}
    \hat{\mathbf{x}_s} = \frac{\sigma_s}{\sigma_t} \mathbf{x}_t - \alpha_s \left(e^{-h_s} - 1\right)\hat{\mathbf{x}_0}
\end{equation}
When using $\gamma$-sampler,  the transition from timestep $t$ to  the next timestep $p$ can be expressed as \Cref{eq:x0clip}, where $s=(1-\gamma)p$.
\begin{equation}
    \mathbf{x}_p = \frac{\alpha_p}{\alpha_s} \hat{\mathbf{x}_s} + \sqrt{1 - \frac{\alpha_p^2}{\alpha_s^2}} \mathbf{z}, \quad \mathbf{z} \in \mathcal{N}(0, I)
    \label{eq:x0clip}
\end{equation}

==> ann/sections/related.tex <==
\section{Related Work}

%\subsection{Diffusion models}
Diffusion models\cite{sohl2015deep, song2019generative, karras2022elucidating} have demonstrated significant advantages in high-quality image synthesis \cite{ramesh2022hierarchical, rombach2022high, dhariwal2021diffusion}, image editing \cite{meng2021sdedit, saharia2022palette, balaji2022ediff}, and specialized tasks such as layout generation \cite{zheng2023layoutdiffusion, wu2024spherediffusion}. However, their multi-step iterative process incurs significant computational costs, hindering real-time applications. Beyond developing faster samplers \cite{song2020denoising,lu2022dpm, lu2022dpm++, zhang2022fast}, there is growing interest in model distillation approaches \cite{sauer2023adversarial, liu2022flow, sauer2024fast, yin2024one}. Among these, distillation methods based on consistency models have proven particularly effective in accelerating processes while preserving output similarity between the original and distilled models.

%\subsection{Consistency models}
\citeauthor{song2023consistency} introduced the concept of consistency models, which emphasize the importance of achieving self-consistency across arbitrary pairs of points on the same probability flow ordinary differential equation (PF-ODE) trajectory \cite{song2020score}. This approach is particularly effective when distilled from a teacher model or when incorporating modules like LCM-LoRA \cite{luo2023lcm}, which can achieve few-step generation with minimal retraining resources.

However, a key limitation of these models is the increased learning difficulty when mapping points further from timestep 0, leading to suboptimal performance when mapping from pure noise in a single step. Phased Consistency Models (PCM) \cite{wang2024phased} address this by dividing the ODE trajectory into multiple sub-trajectories, reducing learning difficulty by mapping each point within a sub-trajectory to its initial point. However, in these methods, each point is mapped to a unique target timestep during distillation, resulting in suboptimal inference when using other timesteps.

Recent advancements, such as Consistency Trajectory Models (CTM) \cite{kim2023consistency} and Trajectory Consistency Distillation (TCD) \cite{zheng2024trajectory}, aim to overcome this by enabling consistency models to perform anytime-to-anytime jumps, allowing all points between timestep 0 and the inference timestep to be used as target timesteps. However, the inclusion of numerous unused target timesteps reduces training efficiency and makes the model less sensitive to fewer-step denoising timesteps.

